Provably Robust Adversarial Examples

We introduce the concept of provably robust adversarial examples for deep neural networks - connected input regions constructed from standard adversarial examples which are guaranteed to be robust to a set of real-world perturbations (such as changes in pixel intensity and geometric transformations). We present a novel method called PARADE for generating these regions in a scalable manner which works by iteratively refining the region initially obtained via sampling until a refined region is certified to be adversarial with existing state-of-the-art verifiers. At each step, a novel optimization procedure is applied to maximize the region's volume under the constraint that the convex relaxation of the network behavior with respect to the region implies a chosen bound on the certification objective. Our experimental evaluation shows the effectiveness of PARADE: it successfully finds large provably robust regions including ones containing $\approx 10^{573}$ adversarial examples for pixel intensity and $\approx 10^{599}$ for geometric perturbations. The provability enables our robust examples to be significantly more effective against state-of-the-art defenses based on randomized smoothing than the individual attacks used to construct the regions.

==> background_old.tex <==
\section{Related Work}
We have chosen to represent our symbolic input regions in terms of convex polytopes, that is, as a set of linear constraints on the input. That allows us to represent complex relationship between the inputs of our neural networks while also allowing for efficient computations with those symbolic regions through the use of Linear Programming (LP) Solvers such as Gurobi[].

To obtain and certify symbolic regions that are provably adversarial we utilize the existing work on neural network verification. In particular, we rely on techniques similar to [14-17, krelu] which employ the triangle ReLU convex relaxation from \cite{lptriangle} and LP Solvers to provably certify output properties of a given neural network for a given symbolic input region. We also utilize the DeepPoly approximation of the triangle relaxation introduced in \cite{deeppoly} to allow us to scale our technique to realistic neural networks with tens of thousands of neurons. In this section we briefly recall how neural network verification works both in the case of the triangle and the DeepPoly relaxations. We also describe the Frank-Wolfe optimization algorithm and how it can be used in conjunction with an LP solver to achieve optimization of an arbitrary objective function constrained to a convex polytope.

\subsection{Neural Network Verification Using the Triangle Convex Relaxation}\label{sec:lp_background}

\input{nn_deeppoly.tex}
\input{relu_triangles.tex}
The verification process using the triangle relaxation works by first encoding the neural network for a specified symbolic input region and then verifying a specified output property such as robustness to adversarial examples for that region. To encode the network the verifier proceeds layer by layer, adding new variables in an LP instance for each encountered neuron alongside constrains that specify what values those variables can take on.

\figref{fig:nn} shows the encoding of a feedforward neural network with ReLU activations and four layers --- an input layer, two hidden layers, and an output layer. All layers in \figref{fig:nn} consist of two neurons, with the ReLU layers being encoded as two layers of two neurons --- one layer for the output of the affine transformation (e.g $x_3$ and $x_4$ at the first hidden layer) and one layer for the result of applying the activation function (e.g $x_5$ and $x_6$ at the first hidden layer).

The encoding process works as follows. The input neurons are constrained to the particular symbolic input region one seeks to verify (the $[-1,1]$-box in \figref{fig:nn}). Neurons that result from affine transformations such as $x_3$ the verifier simply assigns to the respective affine combination of variables on the layer below e.g $x_3=x_1+x_2$. The interesting part of the verification process is the ReLU output encoding. To encode the ReLU output variables one calculates a lower and an upper bound for each ReLU input variable using an LP solver. Based on the lower and upper bound's values we have 3 cases. If the lower bound is positive, that is the value of the input neuron cannot be negative, the verifier assigns the ReLU output variable to the ReLU input variable (e.g $x_9$ in \figref{fig:nn}). Similarly, if the upper bound of the input neuron is negative the verifier assigns the ReLU output variable as being equal to $0$. If the input neuron is not in either of those cases then the output is constrained to be inside a triangle constructed by the neuron's lower and upper bounds (\figref{fig:triangles_a}) giving the triangle relaxation its name. That triangle relaxation for arbitrary $y=\relu(x)$ is given by the following set of constraints:
\begin{align}
&y \geq 0 \label{eq:triangle_lb_0}\\
&y \geq x \label{eq:triangle_lb_x}\\
&y \leq \lambda x + \mu
\end{align}
, with $\lambda=\frac{u}{u-l}$, $\mu=\frac{-lu}{u-l}$ and $u$ and $l$ representing the upper and lower bounds computed by the solver.
For the final robustness verification the verifier performs LP optimizations of the form:
\begin{mini}|l|
{}{x_{true} - x_{adv}}{}{}
\label{eq:final_layer_opt}
\end{mini}, where $x_{true}$ is the output neuron for the correct label and $x_{adv}$ is the output neuron of an adversarial class. If the minimal value obtained by the solver is positive the verification of the input region is successful, that is there is no adversarial examples in the input region.

\subsection{Neural Network Verification Using the DeepPoly Relaxation}

The DeepPoly relaxation introduced in \cite{deeppoly} further loosens the triangle relaxation presented in \secref{sec:lp_background}. It does so by dropping one of the lower bound constraints (\eqref{eq:triangle_lb_0} and \eqref{eq:triangle_lb_x}) from the triangle approximation resulting in the triangles depicted in \figref{fig:triangles_b} and \figref{fig:triangles_c}. The choice which of the two inequalities should be dropped is based on the area of the two triangles --- in particular the DeepPoly relaxation chooses the triangle with the smaller area, thus achieving an overall tighter bound on the output.

Keeping a single upper constraint and a single lower bound constraint on the ReLU output allows the DeepPoly relaxation to avoid relying on LP solvers for computing the lower and upper bounds of individual neurons, as well as, for solving \eqref{eq:final_layer_opt}. Instead, \cite{deeppoly} computes those lower and upper bounds using a backsubstitution algorithm. For all neurons the backsubstitution algorithm computes a lower bound expression $b_i$ and an upper bound expression $c_i$ such that $b_i\le x_i \le c_i$ (\figref{fig:nn}). It does so by repeatedly substituting variables with their upper and lower bound expressions from previous layers until a final lower and upper bound values are computed. 

\figref{fig:nn} shows the results of the backsubstitution algorithm when the process is stopped at the input layer. To demonstrate the operation of the algorithm consider the computation of $c_{11}$. We know $x_{11} = x_9 + x_{10} + 1\leq x_7 + 0.5 \cdot x_8 + 2$, since $x_{10} \leq 0.5 \cdot x_8 + 1$ and $x_9 = x_7$. Analogously, $ x_{7} + 0.5 \cdot x_{8} + 1 =  1.5 \cdot x_{5} + 0.5 \cdot x_{6} + 2 \leq 1.5 \cdot ( 0.5 \cdot x_3  + 1) +  0.5 \cdot ( 0.5 \cdot x_4  + 1) + 2 = 0.75 \cdot x_3 + 0.25 \cdot x_4 + 4 $. Therefore, $x_{11}\leq 0.75 \cdot x_3 + 0.25 \cdot x_4 + 4$. Since, $x_3=x_1+x_2$ and $x_4=x_1-x_2$, we finally arrive at $x_{11} \leq x_1 + 0.5 \cdot x_2 + 4$. Note that if we have box constraints on our input variables, that is constraints of the form $x_{i} \in [l_i,u_i]$ for some $l_i, u_i\in\reals{}$, we can substitute $x_1$ and $x_2$ further in $c_{11}$ to obtain a concrete value for the the upper bound of $x_{11}$. In the case of the network presented in \figref{fig:nn} that bound is $5.5$ obtained at $x_1=x_2=1$. Also note that the $c_{11}$ we obtained is not equal to $c_9 + c_{10} + 1$ and while $c_9 + c_{10} + 1$ is a valid upper bound for $x_{11}$ it is less precise, as it is maximized at $6$ instead of $5.5$.A final note on the DeepPoly verification process is the observation that the backsubstitution algorithm applies to computing \eqref{eq:final_layer_opt}, as well. That is done by calculating the lower and upper expressions of $x_{true}-x_{adv}$. 

By avoiding to explicitly solve the LP problems involved in the verification process the DeepPoly verification algorithm scales to bigger networks. That is the case since LP solvers are based on variations of the Simplex algorithm [] which is an worst-case exponential in the number of LP variables which in the case of neural network verification is exponential in the number of the network's neurons. In contrast, the backsubstitution procedure requires only polynomial number of operations. The price for the computational speed up is payed in terms of the precision of the verifier, as by dropping the constraints we allow more values for the variables involved in the network encoding.
\subsection{The Frank-Wolfe Algorithm}
\input{frankwolf.tex}
The Frank-Wolfe algorithm first presented at \cite{frankwolfe} deals with the optimization problem:
\begin{equation}\label{eq:fw_objective}
       \min_{\boldsymbol{x} \in \mathcal{D}} f(\boldsymbol{x})~,
\end{equation}
where $\mathcal{D}$ is a convex and compact set and $f(\boldsymbol{x})$ is a differentiable L-Lipschitz continuous function. The algorithm is presented at \algref{alg:frankwolfe}. The algorithm is contingent on the optimization used to produce $\boldsymbol{s}_t$ at each step. In the case when $\mathcal{D}$ is a convex polytope one can solve the optimization problem involved using an LP solver. The algorithm also requires the choice of learning rate $\boldsymbol{\gamma}_t$. One can choose 

==> frankwolf.tex <==
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\BREAK}{\STATE \algorithmicbreak}
\begin{algorithm}[tb]
   \caption{Frank–Wolfe Algorithm}
   \label{alg:frankwolfe}
\begin{algorithmic}
   \STATE {\bfseries Input:} initial guess $\boldsymbol{x}_0$, minimum change $\delta$ 
   \FOR{$t=0,1,\hdots$}
       \STATE $\boldsymbol{s}_t = \argmax_{\boldsymbol{s} \in \mathcal{D}} \langle -\nabla f(\boldsymbol{x}_t), \boldsymbol{s}\rangle$
       \STATE
           $\boldsymbol{\gamma}_t = \argmin_{\boldsymbol{\gamma} \in [0, 1]} f(\boldsymbol{x}_t + \boldsymbol{\gamma} \boldsymbol{d}_t)$
       \STATE $\boldsymbol{x}_{t+1} = \boldsymbol{x}_t + \boldsymbol{\gamma}_t \boldsymbol{d}_t$
       \IF{$\|\boldsymbol{x}_{t+1} - \boldsymbol{x}_{t} \|< \delta$}
            \BREAK
       \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

==> nn_decision_boundary_figure/nn_decision_boundary_figure.tex <==
\begin{figure*}[t]
    \centering
    \begin{overpic}[scale=0.12,unit=1mm]{nn_decision_boundary_figure/decision_boundary_nn.pdf}
    	\put(25,30){\textcolor{teal}{$\mathcal{P}$}}
    	\put(42,22){\textcolor{blue}{$\mathcal{A}_c$}}
    \end{overpic}
    \caption{ An example neural network decision boundary in the 2D setting (in blue). The green subregion represents a polyhedral underapproximation $\mathcal{P} \subseteq \mathcal{A}_c$. }
    \vskip -0.1in
\label{fig:nn_decision}
\end{figure*}


==> nn_deeppoly.tex <==
\begin{figure*}
\makeatletter
\pgfdeclaregenericanchor{10 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.1\pgf@xa + 0.9\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{20 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.2\pgf@xa + 0.8\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{30 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.3\pgf@xa + 0.7\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{40 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.4\pgf@xa + 0.6\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{60 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.6\pgf@xa + 0.4\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{80 bottom}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.8\pgf@xa + 0.2\pgf@xb
    \pgf@y=\dimexpr \pgf@yb
}
\pgfdeclaregenericanchor{10 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.1\pgf@xa + 0.9\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\pgfdeclaregenericanchor{20 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.2\pgf@xa + 0.8\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\pgfdeclaregenericanchor{30 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.3\pgf@xa + 0.7\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\pgfdeclaregenericanchor{40 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.4\pgf@xa + 0.6\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\pgfdeclaregenericanchor{60 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.6\pgf@xa + 0.4\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\pgfdeclaregenericanchor{80 top}{
    \pgf@process{\northeast}
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\southwest}
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@x=\dimexpr 0.8\pgf@xa + 0.2\pgf@xb
    \pgf@y=\dimexpr \pgf@ya
}
\makeatother

\centering
\begin{tikzpicture}[font=\tiny\sffamily]
    \node[shape=circle,draw=violet] (A) at (0,0) {$x_{1}$};
    \node[shape=circle,draw=violet] (B) at (0,-1.5) {$x_{2}$};
    \node[shape=circle,draw=gray] (C) at (2.5,0) {$x_{3}$};
    \node[shape=circle,draw=gray] (D) at (2.5,-1.5) {$x_{4}$};
    \node[shape=circle,draw=gray] (E) at (4.75,0) {$x_{5}$};
    \node[shape=circle,draw=gray] (F) at (4.75,-1.5) {$x_{6}$};
    \node[shape=circle,draw=gray] (G) at (7.5,0) {$x_{7}$} ;
    \node[shape=circle,draw=gray] (H) at (7.5,-1.5) {$x_{8}$} ;
     \node[shape=circle,draw=gray] (I) at (10.25,0) {$x_{9}$} ;
    \node[shape=circle,draw=gray] (J) at (10.25,-1.5) {$x_{10}$} ;
    \node[shape=circle,draw=purple] (K) at (13.25,0) {$x_{11}$} ;
    \node[shape=circle,draw=purple] (L) at (13.25,-1.5) {$x_{12}$} ;

    \path [->] (A) edge node[left,above] {1} (C);
    \path [->](B) edge node[left,below] {-1} (D);
    \path [->](A) edge node[pos=0.25,left,above] {1} (D);
    \path [->](B) edge node[pos=0.25,left,above] {1} (C);
    
    \path [->](C) edge node[left,above] {$max(0,x_{3})$} (E);
    \path [->](D) edge node[left,below] {$max(0,x_{4})$} (F);
    
    \path [->] (E) edge node[left,above] {1} (G);
    \path [->](F) edge node[left,below] {-1} (H);
    \path [->](E) edge node[pos=0.25,left,above] {1} (H);
    \path [->](F) edge node[pos=0.25,left,above] {1} (G);
    \path [->](G) edge node[left,above] {$max(0,x_{7})$} (I);
    \path [->](H) edge node[left,below] {$max(0,x_{8})$} (J);
    \path [->] (-1,0) edge node[left,above] {[-1,1]} (A);
    \path [->](-1,-1.5) edge node[left,below] {[-1,1]} (B);
    \path [->] (I) edge node[left,above] {1} (K);
    \path [->](J) edge node[pos=0.25,left,above] {1} (K);
    \path [->] (I) edge node[pos=0.25,left,above] {0} (L);
    \path [->](J) edge node[left,below] {1} (L);

    \coordinate (x1) at (A);
\node at (x1) [above=5.5mm  of x1] { $\begin{aligned} & \langle x_{1} \ge -1 ,\\
							&x_{1} \le 1,\\
							&b_{1} = x_{1}, \\
							&c_{1} = x_{1}\rangle \end{aligned}$ };




\coordinate (x2) at (B);
\node at (x2) [below=5.5mm  of x2] { $\begin{aligned}& \langle  x_{2} \ge -1,\\
							& x_{2} \le 1,\\
							&b_{2} = x_{2}, \\
							&c_{2} = x_{2} \rangle \end{aligned}$ };


 \coordinate (x3) at (C);
\node at (x3) [above=5.5mm  of x3, anchor=60 bottom] { $\begin{aligned}&  \langle x_{3} \ge x_{1} +x_{2},\\
							& x_{3} \le x_{1}+x_{2},\\
							&b_{3} = x_{1} + x_{2}, \\
							&c_{3} = x_{1} + x_{2} \rangle \end{aligned}$ };

\coordinate (x3) at (C);
\node at (x3) [above=2.6mm  of x3] {0};

\coordinate (x4) at (D);
\node at (x4) [below=5.5mm  of x4, anchor=60 top] { $\begin{aligned}& \langle x_{4} \ge x_{1} -x_{2},\\
							& x_{4} \le x_{1}-x_{2},\\
							&b_{4} = x_{1} - x_{2}, \\
							&c_{4} = x_{1} - x_{2} \rangle \end{aligned}$ };

\coordinate (x4) at (D);
\node at (x4) [below=2.6mm  of x4] {0};

\coordinate (x5) at (E);
\node at (x5) [above=5.5mm  of x5,anchor= 40 bottom] { $\begin{aligned}&  \langle x_{5} \ge 0 ,\\
                            &x_{5} \ge x_{3}\textcolor{red}{(\ast)},\\
							& x_{5}\le 0.5 \cdot x_{3} +1,\\
							&b_{5} = 0, \\
							&c_{5} = 0.5\cdot x_{1} + 0.5\cdot x_{2} + 1 \rangle  \end{aligned}$ };


\coordinate (x6) at (F);
\node at (x6) [below=5.5mm  of x6,anchor=40 top] { $\begin{aligned}& \langle x_{6} \ge 0,\\
                            &x_{6} \ge x_{4}\textcolor{red}{(\ast)},\\
							&x_{6} \le 0.5 \cdot x_{4} + 1,\\
							&b_{6} = 0, \\
							&c_{6} = 0.5\cdot x_{1} - 0.5\cdot x_{2} + 1 \rangle \end{aligned}$ };


\coordinate (x7) at (G);
\node at (x7) [above=5.5mm  of x7,anchor=40 bottom] { $\begin{aligned}& \langle x_{7} \ge x_{5} +x_{6},\\
							& x_{7} \le x_{5}+x_{6},\\
							&b_{7} = 0, \\
							&c_{7} = x_{1} + 2 \rangle \end{aligned}$ };

\coordinate (x7) at (G);
\node at (x7) [above=2.6mm  of x7] {0};

\coordinate (x8) at (H);
\node at (x8) [below=5.5mm  of x8,anchor=40 top] { $\begin{aligned}& \langle  x_{8} \ge x_{5} -x_{6},\\
							& x_{8} \le x_{5}-x_{6},\\
							&b_{8} = -0.5\cdot x_{1} - 0.5\cdot x_{2} - 1, \\
							&c_{8} = 0.5\cdot x_{1} + 0.5\cdot x_{2} + 1 \rangle \end{aligned}$ };

\coordinate (x8) at (H);
\node at (x8) [below=2.6mm  of x8] {0};

\coordinate (x9) at (I);
\node at (x9) [above=6mm  of x9,anchor=40 bottom] { $\begin{aligned}&  \langle x_{9} \ge x_{7} ,\\
							& x_{9}\le x_{7},\\
							&b_{9} = 0, \\
							&c_{9} = x_{1} + 2 \rangle \end{aligned}$ };


\coordinate (x10) at (J);
\node at (x10) [below=5.5mm  of x10,anchor=20 top] { $\begin{aligned}& \langle x_{10} \ge 0,\\
                            &x_{10} \ge x_{8}\textcolor{red}{(\ast)},\\
							&x_{10} \le 0.5 \cdot x_{8} + 1,\\
							&b_{10} = 0, \\
							&c_{10} = 0.25\cdot x_{1} + 0.25 \cdot x_{2} + 1.5 \rangle \end{aligned}$ };


\coordinate (x11) at (K);
\node at (x11) [above=6mm  of x11,anchor=30 bottom] { $\begin{aligned}& \langle x_{11} \ge x_{9}+x_{10}+1,\\
							&x_{11} \le x_{9} + x_{10}+1,\\
							&b_{11} = 1, \\
							&c_{11} = x_{1} + 0.5 \cdot x_2 + 4 \rangle \end{aligned}$ };
\coordinate (x11) at (K);
\node at (x11) [above=2.6mm  of x11] {1};

\coordinate (x12) at (L);
\node at (x12) [below=5.5mm  of x12,anchor=30 top] { $\begin{aligned}& \langle x_{12} \ge x_{10},\\
							&x_{12} \le x_{10},\\
							&b_{12} = 0, \\
							&c_{12} = 0.25 \cdot x_{1} + 0.25 \cdot x_{2} + 1.5 \rangle \end{aligned}$ };

\coordinate (x12) at (L);
\node at (x12) [below=2.6mm  of x12] {0};



\end{tikzpicture}
\caption{Encoding of a simple ReLU feedforward neural network using the triangle and the DeepPoly approximations. Constraints marked with $\textcolor{red}{(\ast)}$ are dropped by the DeepPoly approximation. The expressions stored in $b_i$ and $c_i$ for each neuron $x_i$ signify respectively the resulting lower and upper bounds computed by running the DeepPoly backsubstitution algorithm until the input layer. }
\label{fig:nn}
\end{figure*}


==> nn_lp.tex <==
\begin{figure*}[ht!]

\centering
\begin{tikzpicture}[font=\tiny\sffamily]
    \node[shape=circle,draw=violet] (A) at (0,0) {$z_{1}$};
    \node[shape=circle,draw=violet] (B) at (0,-1.5) {$z_{2}$};
    \node[shape=circle,draw=gray] (C) at (2,0) {$z_{3}$};
    \node[shape=circle,draw=gray] (D) at (2,-1.5) {$z_{4}$};
    \node[shape=circle,draw=gray] (E) at (4,0) {$z_{5}$};
    \node[shape=circle,draw=gray] (F) at (4,-1.5) {$z_{6}$};
    \node[shape=circle,draw=gray] (G) at (6,0) {$z_{7}$} ;
    \node[shape=circle,draw=gray] (H) at (6,-1.5) {$z_{8}$} ;
     \node[shape=circle,draw=gray] (I) at (8,0) {$z_{9}$} ;
    \node[shape=circle,draw=gray] (J) at (8,-1.5) {$z_{10}$} ;
    \node[shape=circle,draw=purple] (K) at (10,0) {$z_{11}$} ;
    \node[shape=circle,draw=purple] (L) at (10,-1.5) {$z_{12}$} ;

    \path [->] (A) edge node[left,above] {$1$} (C);
    \path [->](B) edge node[left,below] {$-1$} (D);
    \path [->](A) edge node[pos=0.25,left,above] {$1$} (D);
    \path [->](B) edge node[pos=0.25,left,above] {$1$} (C);
    
    \path [->](C) edge node[left,above] {$\max(0,z_{3})$} (E);
    \path [->](D) edge node[left,below] {$\max(0,z_{4})$} (F);
    
    \path [->] (E) edge node[left,above] {$1$} (G);
    \path [->](F) edge node[left,below] {$-1$} (H);
    \path [->](E) edge node[pos=0.25,left,above] {$1$} (H);
    \path [->](F) edge node[pos=0.25,left,above] {$1$} (G);
    \path [->](G) edge node[left,above] {$\max(0,z_{7})$} (I);
    \path [->](H) edge node[left,below] {$\max(0,z_{8})$} (J);
    \path [->] (-1,0) edge node[left,above] {$[-1,1]$} (A);
    \path [->](-1,-1.5) edge node[left,below] {$[-1,1]$} (B);
    \path [->] (I) edge node[left,above] {$1$} (K);
    \path [->](J) edge node[pos=0.25,left,above] {$1$} (K);
    \path [->] (I) edge node[pos=0.25,left,above] {$0$} (L);
    \path [->](J) edge node[left,below] {$1$} (L);

    \coordinate (x1) at (A);
\node at (x1) [above=5.5mm  of x1] { $\begin{aligned} & \langle z_{1} \ge -1 ,\\
							&z_{1} \le 1,\\
						    &\tilde{g}_1=0.5,\\
                            &g_1^*=1 \rangle \end{aligned}$ };




\coordinate (x2) at (B);
\node at (x2) [below=5.5mm  of x2] { $\begin{aligned}& \langle  z_{2} \ge -1,\\
							& z_{2} \le 1,\\
						    &\tilde{g}_2=-0.5,\\
                            &g_2^*=-1  \rangle \end{aligned}$ };


 \coordinate (x3) at (C);
\node at (x3) [above=5.5mm  of x3] { $\begin{aligned}&  \langle z_{3} = z_{1} +z_{2}, \\
                                     &\tilde{g}_3=0,\\
                                     &g_3^*=0 \rangle \end{aligned}$ };

\coordinate (x3) at (C);
\node at (x3) [above=2.6mm  of x3] {$0$};

\coordinate (x4) at (D);
\node at (x4) [below=5.5mm  of x4] { $\begin{aligned}& \langle z_{4} = z_{1} -z_{2}, \\
                                     &\tilde{g}_4=1,\\
                                     &g_4^*=2 \rangle \end{aligned}$ };

\coordinate (x4) at (D);
\node at (x4) [below=2.6mm  of x4] {$0$};

\coordinate (x5) at (E);
\node at (x5) [above=5.5mm  of x5] { $\begin{aligned}&  \langle z_{5} \ge 0 ,\\
                            & z_{5}\ge z_{3},\\
							& z_{5}\le 0.5 \cdot z_{3} +1,\\
							&\tilde{g}_5=1,\\
                            &g_5^*=1  \rangle  \end{aligned}$ };


\coordinate (x6) at (F);
\node at (x6) [below=5.5mm  of x6] { $\begin{aligned}& \langle z_{6} \ge 0,\\
                            &z_{6}\ge z_{4},\\
							&z_{6} \le 0.5 \cdot z_{4} + 1,\\
							&\tilde{g}_6=1,\\
                            &g_6^*=2 \rangle \end{aligned}$ };


\coordinate (x7) at (G);
\node at (x7) [above=5.5mm  of x7] { $\begin{aligned}& \langle z_{7} = z_{5} +z_{6},\\
							&\tilde{g}_7=2,\\
                            &g_7^*=3 \rangle \end{aligned}$ };

\coordinate (x7) at (G);
\node at (x7) [above=2.6mm  of x7] {$0$};

\coordinate (x8) at (H);
\node at (x8) [below=5.5mm  of x8] { $\begin{aligned}& \langle  z_{8} = z_{5} -z_{6},\\
							&\tilde{g}_8=0,\\
                            &g_8^*=-1 \rangle \end{aligned}$ };

\coordinate (x8) at (H);
\node at (x8) [below=2.6mm  of x8] {$0$};

\coordinate (x9) at (I);
\node at (x9) [above=6mm  of x9] { $\begin{aligned}&  \langle z_{9} = z_{7} ,\\
							&\tilde{g}_9=2,\\
                            &g_9^*=3 \rangle \end{aligned}$ };


\coordinate (x10) at (J);
\node at (x10) [below=5.5mm  of x10] { $\begin{aligned}& \langle z_{10} \ge 0,\\
                            &z_{10} \ge x_8,\\
							&z_{10} \le 0.5 \cdot z_{8} + 1,\\
							&\tilde{g}_{10}=1,\\
                            &g_{10}^*=0.5 \rangle \end{aligned}$ };


\coordinate (x11) at (K);
\node at (x11) [above=6mm  of x11] { $\begin{aligned}& \langle z_{11} = z_{9}+z_{10}+1,\\
							&\tilde{g}_{11}=4,\\
                            &g_{11}^*=4.5 \rangle \end{aligned}$ };
\coordinate (x11) at (K);
\node at (x11) [above=2.6mm  of x11] {$1$};

\coordinate (x12) at (L);
\node at (x12) [below=5.5mm  of x12] { $\begin{aligned}& \langle z_{12} = z_{10},\\
							&\tilde{g}_{12}=1,\\
                            &g_{12}^*=0.5 \rangle \end{aligned}$ };

\coordinate (x12) at (L);
\node at (x12) [below=2.6mm  of x12] {$0$};



\end{tikzpicture}
\vspace*{-3mm}
\caption{Fast counterexample evaluation on a ReLU based fully-connected network with four layers. The values $\tilde{g}_i$ approximate the worst-case neuron values of the candidate $(0.5, -0.5)$. The values $g^*$ correspond to the worst possible abstract counterexample $(1,-1)$. }
\label{fig:nn_lp}
\vskip -0.1in
\end{figure*}


==> overview_figure/overview_figure.tex <==
\begin{figure*}[t]
\vskip -3em
\centering
\def \boxsize {60mm}
\def \minw {39mm}
\def \minh {55mm}
\makeatletter
\newcommand{\stepbox}[6]{
	\ifblank{#1} {\node}{node} (#2)
	[draw=black!60, fill=black!05, rectangle, rounded corners=2pt,
	minimum width=\minw, minimum height=\minh,anchor=north west, #3] at (#4, #5) {#6}
}
\makeatother
\makeatletter
\newcommand{\gettikzx}[2]{%
	\tikz@scan@one@point\pgfutil@firstofone#1\relax
	\edef#2{\the\pgf@x}%
}
\makeatother
\makeatletter
\newcommand{\gettikzy}[2]{%
	\tikz@scan@one@point\pgfutil@firstofone#1\relax
	\edef#2{\the\pgf@y}%
}
\makeatother

\makeatletter      
\newcommand{\getAngle}[3]{%
	\pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}
	{\pgfpointanchor{#2}{center}}
	\pgfmathsetmacro{#3}{\pgfmathresult}
}
\makeatother

\makeatletter      
\newcommand{\getDistance}[4]{%
	\getAngle{#2}{#1}{\anglep}
	\getAngle{#2}{#3}{\anglel}
	\gettikzx{(#1)}{\vx}
	\gettikzy{(#1)}{\vy}
	\gettikzx{(#2)}{\lx}
	\gettikzy{(#2)}{\ly}
	\pgfmathveclen{\vx-\lx}{\vy-\ly}
	\pgfmathsetmacro{\lenp}{\pgfmathresult}
	\pgfmathparse{sin(\anglep - \anglel)*\lenp}
	\edef#4{\pgfmathresult pt}
}
\makeatother

\makeatletter      
\newcommand{\myoffsetBy}[6]{%
	\gettikzx{(#1)}{\vxo}
	\gettikzy{(#1)}{\vyo}
	\gettikzx{(#2)}{\lx}
	\gettikzy{(#2)}{\ly}
	\pgfmathveclen{\vxo-\lx}{\vyo-\ly}
	\pgfmathsetmacro{\leno}{\pgfmathresult}
	
	\gettikzx{(#3)}{\vxt}
	\gettikzy{(#3)}{\vyt}
	\pgfmathveclen{\vxt-\lx}{\vyt-\ly}
	\pgfmathsetmacro{\lent}{\pgfmathresult}
	
	\pgfmathparse{#4}
	\edef#5{\pgfmathresult pt}
	\pgfmathsetmacro{\offseto}{\pgfmathresult}
	\pgfmathparse{#4/\leno*\lent}
	\edef#6{\pgfmathresult pt}
	\pgfmathsetmacro{\offsett}{\pgfmathresult}
}
\makeatother

\newcommand{\subfigtitle}[3]{
	\begin{scriptsize}{
		\begin{tabular}{l@{\hspace{1em}}l@{}}
			#1. & #2\\
			& #3
		\end{tabular}
	}\end{scriptsize}
}
\scalebox{0.8}{\begin{tikzpicture}[font=\small\sffamily]
	\tikzset{>=latex}
  	\stepbox{}{step1}{minimum width=\minw*2 +5mm}{0}{0}{};
  	\path let
  	\p1=(step1.north east)
  	in
  	\stepbox{True}{step21}{minimum width=\minw*2 + 5mm}{\x1 + 5mm}{0}{};
	
	\node[anchor=west] (over1) at ($(step1.west) + (2mm, 0)$) {\input{overview_figure/overapprox1.tex}};
	\node[anchor=east] (over2) at ($(step1.east) + (-2mm, 0)$) {\input{overview_figure/overapprox2.tex}};
	\node[anchor=west] (under1) at ($(step1.east) + (7mm, 0)$) {\input{overview_figure/underapprox1.tex}};
	\node[anchor=east] (under2) at ($(step21.east) + (-2mm, 0)$) {\input{overview_figure/underapprox2.tex}};
	
	\node[anchor=north] (poly0) at ($(step1.north) + (0, -2mm)$) {\begin{normalsize}Overapproximation Box\end{normalsize}};
	\node[anchor=north] (poly0) at ($(step21.north) + (0, -2mm)$) {\begin{normalsize}Underapproximation Box\end{normalsize}};
	
	\node[anchor=north] (poly0) at ($(over1.south) + (-2mm, 1mm)$)
	{\subfigtitle{1}{Generate samples}{by attacking the network}};
	\node[anchor=north] (poly0) at ($(over2.south) + (-3mm, 1mm)$)
	{\subfigtitle{2}{Generate an overapproximation}{ box from samples}};
	\node[anchor=north] (poly0) at ($(under1.south) + (-1mm, 1mm)$) {\subfigtitle{3}{Try to verify the network and}{create a target hyperplane}};
	\node[anchor=north] (point4) at ($(under2.south) + (-2mm, 1mm)$) {\subfigtitle{4}{Adjust the target hyperplane's}{bias and shrink box accordingly}};
	
	\path[->] ($(over1.east) + (2mm,0)$) edge node [below] {\begin{footnotesize}Fit Box\end{footnotesize}} ($(over2.west) + (3mm,0)$);
	\path[->] ($(over2.east) + (0.5mm,0)$) edge node [below] {\begin{footnotesize}Initialize\end{footnotesize}} ($(under1.west) + (3mm,0)$);
	
	\path[->] ($(under1.east)+(2mm,-2mm)$) edge[bend right] node [below] {\begin{footnotesize}Adjust Box\end{footnotesize}} ($(under2.west)+(2mm,-2mm)$);
	\path[->] ($(under2.west)+(2mm,2mm)$) edge[bend right] node [above] {\begin{footnotesize}Get Target\end{footnotesize}} ($(under1.east)+(2mm,2mm)$);

\end{tikzpicture}}
\vskip -0.1in
\caption{Overview of \tool{}. The green triangle denoted $\mathcal{T}$ represents the ground truth adversarial region and the red crosses represent the attacks obtained by \advalg{}. The dashed blue and violet dotted rectangles denoted $\mathcal{O}$ and  $\mathcal{U}$, represent the fitted overapproximation and underapproximation boxes, respectively. The solid black lines represent hyperplanes generated by the verification procedure, while their dash-dotted counterparts represent the hyperplanes after bias-adjustment. The arrows going out of the hyperplanes represent the direction of their corresponding half-spaces.}
\vskip -0.8em
\label{fig:overview}
\end{figure*}


==> related.tex <==
\section{Related Work}
Our work is closely related to previous work on robust adversarial examples, such as ~\citep{pgd, athalye:18b,audioemp} but differs in that the previous work does not generate any continuous regions that is provably robust like our work does and instead tries to find a single adversarial image, whose neighbourhood is empirically adversarial. 

Additionally, our work relates to previous work on generating neural network input regions from output conditions. This includes the work of \citet{Dathathri:19} that uses symbolic interpolation to compute both an under- and an overapproximation of the set of inputs for which a given output property holds and the work of \citet{armando} and \citet{corina} that explore linear regions specified by the activation patterns of the neurons in the network to generate robust regions. We note that these works do not scale to the input dimensions involved in our $L_\infty$ experiments and do not support geometric transformations due to their reliance on the piecewise-linearity of the network operations. In contrast, our robust adversarial example generation scales to larger networks, larger input parameter spaces and can be easily extended to work with many existing robust certification methods that certify diverse set of perturbations.


==> relu_triangles.tex <==
\begin{figure*}
\centering

\begin{tikzpicture}
\coordinate (l1) at (-1,0);
\coordinate (u1) at (1,1);
\coordinate (v1) at (1,0);
\coordinate (o1) at (0,0);
\coordinate (startx1) at (-1.3,0);
\coordinate (endx1) at (1.5,0);
\coordinate (starty1) at (0,-1);
\coordinate (endy1) at (0,1.6);
\coordinate (startl1) at (-1,-1);
\coordinate (endl1) at (-1,1);
\coordinate (startu1) at (1,-1);
\coordinate (endu1) at (1,1);

\def\distx{5}
\def\disty{4}
\def\height{-0.9}
\def\width{1.1}

\coordinate (l2) at ($(l1) + (\distx,0)$);
\coordinate (u2) at ($(u1) + (\distx,0)$);
\coordinate (v2) at ($(startl1) + (\distx,0)$);
\coordinate (o2) at ($(0,0) + (\distx,0)$);
\coordinate (startx2) at ($(startx1) + (\distx,0)$);
\coordinate (endx2) at ($(endx1) + (\distx,0)$);
\coordinate (starty2) at ($(starty1)+(\distx,0)$);
\coordinate (endy2) at ($(endy1) + (\distx,0)$);
\coordinate (startl2) at ($(startl1) + (\distx,0)$);
\coordinate (endl2) at ($(endl1) + (\distx,0)$);
\coordinate (startu2) at ($(startu1) + (\distx,0)$);
\coordinate (endu2) at ($(endu1) + (\distx,0)$);

\coordinate (l3) at ($(l1) + (-\distx,0)$);
\coordinate (u3) at ($(u1) + (-\distx,0)$);
\coordinate (v3) at ($(0,0) + (-\distx,0)$);
\coordinate (startx3) at ($(startx1) + (-\distx,0)$);
\coordinate (endx3) at ($(endx1) + (-\distx,0)$);
\coordinate (starty3) at ($(starty1)+(-\distx,0)$);
\coordinate (endy3) at ($(endy1) + (-\distx,0)$);
\coordinate (startl3) at ($(startl1) + (-\distx,0)$);
\coordinate (endl3) at ($(endl1) + (-\distx,0)$);
\coordinate (startu3) at ($(startu1) + (-\distx,0)$);
\coordinate (endu3) at ($(endu1) + (-\distx,0)$);

\coordinate (l4) at ($(l1) + (\distx,\disty)$);
\coordinate (u4) at ($(u1) + (\distx,\disty)$);
\coordinate (v4) at ($(1,0.5) + (\distx,\disty)$);
\coordinate (w4) at ($(-1,-0.5) + (\distx,\disty)$);
\coordinate (o4) at ($(0,0) + (\distx,\disty)$);
\coordinate (startx4) at ($(startx1) + (\distx,\disty)$);
\coordinate (endx4) at ($(endx1) + (\distx,\disty)$);
\coordinate (starty4) at ($(starty1)+(\distx,\disty)$);
\coordinate (endy4) at ($(endy1) + (\distx,\disty)$);
\coordinate (startl4) at ($(startl1) + (\distx,\disty)$);
\coordinate (endl4) at ($(endl1) + (\distx,\disty)$);
\coordinate (startu4) at ($(startu1) + (\distx,\disty)$);
\coordinate (endu4) at ($(endu1) + (\distx,\disty)$);


\draw[->] (startx3) --(endx3);
\draw[->] (starty3) --(endy3);
\draw (l3)[thick] --(u3);
\draw (u3)[thick] --(v3);
\draw (l3)[thick] --(v3);
\draw (startl3)  --(endl3);
\draw (startu3) --(endu3);

\draw[fill=lightgray]  (l3) -- (v3) -- (u3) -- cycle;

\coordinate (X3) at (endx3);
\node at (X3) [right=0.1mm  of X3] { $x_{i}$};

\coordinate (Y3) at (endy3);
\node at (Y3) [above=0.1mm  of Y3] { $x_{j}$};

\coordinate (P3) at ($0.4*(endu3) + 0.6*(startu3)$);
\node at (P3) [right=0.1mm  of P3] { $u_{i}$};

\coordinate (R3) at ($0.4*(endl3) + 0.6*(startl3)$);
\node at (R3) [left=0.1mm  of R3] { $l_{i}$};

\coordinate (Q3) at ($(endy3)+(-1.08,-1.3)$);
\node at (Q3) [right=0.1mm  of Q3, rotate=26] { $x_{j}=\lambda \cdot x_{i} + \mu$};


\coordinate (S3) at ($(v3)+(0.25,-0.05)$);
\node at (S3) [right=0.1mm  of S3,rotate=45] { $x_{j}=x_{i}$};
\coordinate (O3) at (starty3);
\node at (O3) [below=0.1mm  of O3] {  (a) \label{fig:test-foo}};
\subfloat[\label{fig:triangles_a}]

\draw[->] (startx1) --(endx1);
\draw[->] (starty1)  --(endy1);
\draw (l1)[thick] --(u1);
\draw (l1)[thick] --(v1);
\draw (startl1) --(endl1);
\draw (startu1) --(endu1);

\draw[fill=lightgray]  (l1) -- (v1) -- (u1) -- cycle;

\coordinate (X1) at (endx1);
\node at (X1) [right=0.1mm  of X1] { $x_{i}$};

\coordinate (Y1) at (endy1);
\node at (Y1) [above=0.1mm  of Y1] { $x_{j}$};


\coordinate (P1) at ($0.4*(endu1) + 0.6*(startu1)$);
\node at (P1) [right=0.1mm  of P1] { $u_{i}$};

\coordinate (R1) at ($0.4*(endl1) + 0.6*(startl1)$);
\node at (R1) [left=0.1mm  of R1] { $l_{i}$};

\coordinate (Q1) at ($(endy1)+(-1.08,-1.3)$);
\node at (Q1) [right=0.1mm  of Q1, rotate=26] { $x_{j}=\lambda \cdot x_{i} + \mu$};

\coordinate (O1) at (starty1);
\node at (O1) [below=0.1mm  of O1] {  (b) };
\subfloat[\label{fig:triangles_b}]

\draw[->] (startx2) --(endx2);
\draw[->] (starty2) --(endy2);
\draw (l2)[thick] --(u2);
\draw (u2)[thick] --(v2);
\draw (startl2)  --(endl2);
\draw (startu2) --(endu2);

\draw[fill=lightgray]  (l2) -- (v2) -- (u2) -- cycle;

\coordinate (X2) at (endx2);
\node at (X2) [right=0.1mm  of X2] { $x_{i}$};

\coordinate (Y2) at (endy2);
\node at (Y2) [above=0.1mm  of Y2] { $x_{j}$};

\coordinate (P2) at ($0.4*(endu2) + 0.6*(startu2)$);
\node at (P2) [right=0.1mm  of P2] { $u_{i}$};

\coordinate (R2) at ($0.4*(endl2) + 0.6*(startl2)$);
\node at (R2) [left=0.1mm  of R2] { $l_{i}$};

\coordinate (Q2) at ($(endy2)+(-1.08,-1.3)$);
\node at (Q2) [right=0.1mm  of Q2, rotate=26] { $x_{j}=\lambda \cdot x_{i} + \mu$};


\coordinate (S2) at ($(v2)+(0.3,0)$);
\node at (S2) [right=0.1mm  of S2, rotate=45] { $x_{j}=x_{i}$};

\coordinate (O2) at (starty2);
\node at (O2) [below=0.1mm  of O2] {  (c) };
\subfloat[\label{fig:triangles_c}]










\end{tikzpicture}
\vspace*{-3mm}
\caption{Convex approximations for the ReLU function: (a) shows the convex approximation with the minimum area in the input-output plane, (b) and (c) show the two convex approximations proposed in this paper. In the figure, $\lambda= u_{i}/(u_{i}-l_{i})$ and $\mu=-l_{i}u_{i}/(u_{i}-l_{i})$.}
\label{fig:triangles}
\end{figure*}


==> theorem_figure/theorem_23.tex <==
\begin{tikzpicture}
[   declare function={
	mu1=1;
	mu2=2;
	sigma1=0.5;
	sigma2=1;
	normal(\m,\s)=1/(2*\s*sqrt(pi))*exp(-(x-\m)^2/(2*\s^2));
	bivar(\ma,\sa,\mb,\sb)=
	1/(2*pi*\sa*\sb) * exp(-((x-\ma)^2/\sa^2 + (y-\mb)^2/\sb^2))/2;
	mybivar(\x,\y,\ma,\sa,\mb,\sb)=
	1/(2*pi*\sa*\sb) * exp(-((\x-\ma)^2/\sa^2 + (\y-\mb)^2/\sb^2))/2;   
	invgauss(\a,\b) = sqrt(-2*ln(\a))*cos(deg(2*pi*\b));}]

\begin{axis}[
width=0.4\paperwidth,
xlabel style={below right},
ylabel style={above left},
xmin=-0.5,
xmax=8.5,
ymin=-0.5,
ymax=8.5,
ticks=none,
axis lines=none
]
\coordinate (O) at (axis cs:0,0);
\coordinate (X) at (axis cs:1,0);
\coordinate (Y) at (axis cs:0,1);
\addplot[scatter,clip=true, clip marker paths=true,
only marks, mark=-, samples=100,
scatter/classes={0={mark=-,red},
	1={mark=,red}},point meta=int(1)<0,
]({1*rand + 6.5},{4*rand + 4});

\addplot[scatter,clip=true, clip marker paths=true,
only marks, mark=-, samples=100,
scatter/classes={0={mark=+,green},
	1={mark=,red}},point meta=int(1)<0,
]({1.9*rand + 2},{2.4*rand + 2.5});
\end{axis}
\def\centerarc[#1](#2)(#3:#4:#5)%
{ \filldraw[#1] ($(#2)$) -- ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5) -- cycle }
\begin{scope}[x={($(X)-(O)$)}, y={($(Y)-(O)$)}, shift={(O)}]
\draw[blue,thick] (0,0) rectangle (8,8);
\draw[red,thick] (0,0) rectangle (5,5);
\fill[fill=orange,opacity=.5] (4,0) rectangle (5,5);
\draw[green,thick,opacity=0] (7,6.2) -- (7,0)  node[below,black] {$u^i_2$}; %
\draw[decorate,decoration={brace,amplitude=5pt,raise=0.5pt,mirror},black,thick] (4,0) -- (5,0) node[midway,below,black, yshift=-2.5] {$\epsilon_i$};
\draw[red,thick] (4,0) -- (5,0);
\draw[red,thick] (0,0) rectangle (0,5) node[midway,left,black] {$\sigma$};
\filldraw[black] (4,0) circle (2pt)  node[anchor=south east, black] {$p$};
\draw[black,thick,dashed] (4.1,-0.5) -- (3,8.5) node[anchor=south east, black]{$h_{i}$};
\draw[black,thick,dashed] (5,-0.5) -- (3.95,8.5);
\filldraw[green] (4.4,5) circle (2pt) node[anchor=south west, black] {$p^{\min}_{1}$};
\draw[decorate,decoration={brace,amplitude=5pt,raise=0.5pt, mirror},black,thick] (3.4,5) -- (4.4,5) node[midway,below,black, yshift=-2.5] {$\epsilon_{i}$};

\draw[decorate,decoration={brace,amplitude=5pt,raise=0.3pt, mirror},black,thick] (4.4,5) -- (5,5) node[midway,below,black, yshift=-2.5] {$\delta$};
\draw[red,thick,dashed] (4,-0.5) -- (4,8.5);
\draw[red,->,thick] ( 4, 0 ) -- (1,0);
\draw[->,thick] ( 4,0 ) -- (1.1,-0.8);
\filldraw[blue] (3.4,5) circle (2pt) node[anchor=south east, black] {$x^{\min}_i$};
\filldraw[red] (5,0) circle (2pt) node[anchor=south west, black] {$p^{\max}_{2}$};
\centerarc[fill opacity=0.5,fill=blue](4,0)(180:195:1.8) node[midway,left=0.8,black, opacity=1] {$\alpha$};
\end{scope}
\end{tikzpicture}

==> theorem_figure/theorem_24.tex <==
\begin{tikzpicture}
[   declare function={
    mu1=1;
    mu2=2;
    sigma1=0.5;
    sigma2=1;
    normal(\m,\s)=1/(2*\s*sqrt(pi))*exp(-(x-\m)^2/(2*\s^2));
    bivar(\ma,\sa,\mb,\sb)=
        1/(2*pi*\sa*\sb) * exp(-((x-\ma)^2/\sa^2 + (y-\mb)^2/\sb^2))/2;
    mybivar(\x,\y,\ma,\sa,\mb,\sb)=
        1/(2*pi*\sa*\sb) * exp(-((\x-\ma)^2/\sa^2 + (\y-\mb)^2/\sb^2))/2;   
    invgauss(\a,\b) = sqrt(-2*ln(\a))*cos(deg(2*pi*\b));}]
 
\begin{axis}[
width=0.4\paperwidth,
xlabel style={below right},
ylabel style={above left},
xmin=-0.5,
xmax=8.5,
ymin=-0.5,
ymax=8.5,
ticks=none,
axis lines=none
]
\coordinate (O) at (axis cs:0,0);
\coordinate (X) at (axis cs:1,0);
\coordinate (Y) at (axis cs:0,1);
\addplot[scatter,clip=true, clip marker paths=true,
only marks, mark=-, samples=100,
scatter/classes={0={mark=+,green},
	1={mark=,red}},point meta=int(1)<0,
]({2.4*rand + 2.5},{2.4*rand + 2.5});
\addplot[scatter,clip=true, clip marker paths=true,
only marks, mark=-, samples=30,
scatter/classes={0={mark=-,red},
	1={mark=,red}},point meta=int(1)<0,
]({0.4*rand + 6.5},{3*rand + 3.1});
\end{axis}
\begin{scope}[x={($(X)-(O)$)}, y={($(Y)-(O)$)}, shift={(O)}]
\draw[blue,thick] (0,0) rectangle (8,8);
\draw[red,thick] (0,0) rectangle (5,5);
\draw[black,thick,dashed,opacity=0] (4.1,-0.5) -- (3,8.5) node[above, black] {$l$}; %
\draw[green,thick] (7,6.2) -- (7,0)  node[below,black] {$u_{i}^2$};
\draw[green,thick] (7,6.2) -- (0,6.2) node[left,black] {$u_{i}^1$};
\draw[red,thick] (5,0) rectangle (6,0);
\draw[red,thick] (0,0) rectangle (0,5) node[midway,left,black] {$\sigma$};
\fill[fill=orange,opacity=.5] (5,0) rectangle (6,6.2);
\filldraw[black] (5.8,2.5) circle (2pt) node[anchor=south east, black] {$p$};
\draw[black,thick,dashed] (5.8,-0.5) -- (5.8,8.5) node[anchor=south west, black]{$h_{i+1}$};
\end{scope}
\end{tikzpicture}

==> theorem_figure/theorem_fig.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[Illustration of \lemmaref{lm:hp_vol_shrink_lemma}.]{\label{fig:theorem23}\input{theorem_figure/theorem_23}}
    \hspace*{3mm}
    \subfigure[Illustration of \thref{th:it_progress_theorem}.]{\label{fig:theorem24}\input{theorem_figure/theorem_24}}
    \vspace*{-3mm}
    \caption{ 
Illustrations of the proofs in \secref{sec:theory}. In both subfigures, the blue box represents the input space hyperbox $\mathcal{I}$, the red box represents $\mathcal{A}_c$ and the orange shaded region represents the volume from which we sample $p$. Additionally, in both subfigures, we represent the rest of the positive and negative samples in $\mathcal{D}_i$ with green pluses and red minuses, respectively. In (a), the angle $\alpha$ represents the maximum allowed angle between the normals of $h_i$ and the decision boundary of $\mathcal{A}_c$. The blue dot represents the point with the worst possible horizontal error $x^{\min}_i$ when a point is sampled in the orange region. . In (b), the green box represents the region $\mathcal{P}_i$ to which $h_{i+1}$ is added.
}
    \vskip -0.1in
\label{fig:proof}
\end{figure*}


==> theory.tex <==
\section{Hardness of Generating Symbolic Adversarial Examples}\label{sec:theory}
Neural networks are often applied to high-dimensional input domains, such as images and audio, which are particularly vulnerable to adversarial examples, as demonstrated by \citet{khoury2018geometry,gilmer2018adversarial}. Therefore, it is crucial that algorithms for creating symbolic adversarial regions scale to high-dimensional inputs. In this work, we focus on a family of algorithms that compute symbolic regions via a greedy approach. Our experimental observations in \secref{sec:eval} confirm that such algorithms are more scalable and precise than other known alternatives \citep{armando,corina} that generate regions by enumerating all paths in the network which are exponential in the number of neurons for ReLU based networks considered in our work. Combining these regions for producing a single convex symbolic region again has exponential complexity in the number of input dimensions.
In this section, we provide a theoretical analysis of the complexity of greedily generating optimal (in terms of volume) polyhedral symbolic adversarial examples. 
Our analysis shows that this has exponential complexity in the number of input dimensions.

 




Let $\mathcal{C}$ be the set of all binary classifiers with continuous decision boundaries that assign labels from $\{-1,1\}$ to a connected subspace $\mathcal{I}$ of $\reals{d}$. Note that all neural networks with continuous activation functions are in $\mathcal{C}$. Let $f\in\mathcal{C}$ be a ground-truth binary classifier which we want to approximate using a learning algorithm. The algorithm creates an approximation $c\in\mathcal{C}$ of $f$ based on a finite dataset of training samples $\mathcal{D}=\{(x_i,f(x_i))\}_{i=1,\dots, m}$. Here, the $x_i$'s are drawn from an unknown input probability distribution $P$ on $\mathcal{I}$. To simplify analysis, we assume that the approximate classifier $c$ correctly classifies all the points in $\mathcal{D}$.

\input{nn_decision_boundary_figure/nn_decision_boundary_figure}

We call the region $\mathcal{A}_c=\{ x\in \mathcal{I} \mid c(x) \neq f(x)\}$ the adversarial region of $c$. We note that $\mathcal{A}_c$ does not contain any points from $\mathcal{D}$. %
$\mathcal{A}_c$ is usually a disjoint union of connected regions (instead of being a single connected region). \figref{fig:nn_decision} shows $\mathcal{A}_c$ (in blue) for a ReLU based neural network. The green region in the figure represents a polyhedral approximation $\mathcal{P} \subseteq \mathcal{A}_c$. %
Since $\mathcal{P}$ is a polyhedron, it must be contained entirely within one of the connected subregions of $\mathcal{A}_c$.
 Note that the algorithms developed in this paper can be applied to generate multiple regions $\mathcal{P}$ for each subregion of $\mathcal{A}_c$. However, this is generally computationally prohibitive for neural networks, where many such regions exist. To simplify notation, we use $\mathcal{A}_c$ to refer to the connected subregion containing $\mathcal{P}$ for the remainder of this section.

Our algorithms create $\mathcal{P}$ iteratively by cutting volume away from $\mathcal{I}$ until $\mathcal{P}\subseteq \mathcal{A}_c$. i.e., we generate a sequence of polyhedra $\{\mathcal{P}_i\}_{i=0,\dots ,m}$ where $\mathcal{P}_{0}= \mathcal{I}$ and $\mathcal{P}=\mathcal{P}_{m}\subseteq \mathcal{A}_c$. Each polyhedron in the sequence is created from the previous one by intersecting it with an additional half-space constraint $h_i:a_{i} x+ b_i \leq 0$  with parameters $a_{i} \in \mathds{R}^d, b_i \in \mathds{R}$. The linear classifier $h_i$ is estimated from a separate dataset $\mathcal{D}_i$, sampled using the input distribution $P$ and evaluated using $f$. 
In order to fit the linear classifiers $h_i$ we require each dataset $\mathcal{D}_i$ to contain both positive samples ($x$ such that $f(x)\neq c(x)$) and negative samples ($x$ such that $f(x)= c(x)$).

A positive sample $x$ is correctly classified by $h_i$ if $a_{i} x+ b_i \leq 0$ --- that is, $h_i$ keeps it in $\mathcal{P}_{i}$, and incorrectly classified otherwise.
Similarly, a negative sample $x$ is correctly classified by $h_i$ if $a_{i} x + b_i \geq 0$ --- that is, $h_i$ removes it from $\mathcal{P}_{i}$, and incorrectly classified otherwise. To simplify notations, we assume that samples $x$, for which $a_{i} x + b_i = 0$ can be regarded as both correctly classified and missclassified. We use the volume ratio $\frac{\vol(\mathcal{P})}{\vol(\mathcal{A}_c)}$ to quantify the effectiveness of our algorithms.



For the remainder of this section, we focus on analyzing the aforementioned family of algorithms under a simplified setting to intuitively demonstrate the inherent hardness of computing symbolic adversarial examples and thereby motivating the need for the methods developed in this paper. We will show that our problem is hard even in this simplified setting; in the more general setting, our problem may be even harder.

We choose a setting where we have an analytic characterization of the decision boundary learned by the model and thus an explicit formula for $\vol(\mathcal{A}_{c})$. We choose $\mathcal{A}_c$ to be a $d$-dimensional hyperbox $[0,\sigma]^d$ for some $\sigma\in (0,1)$ with $d$ decision boundaries. The $i^\mathit{th}$ decision boundary of our chosen $\mathcal{A}_c$ is $a_{i}^\text{best} \cdot x + b_{i}^\text{best} = 0$ with $a_{i}^\text{best}=e_{i}$ and $b_{i}^\text{best}=-\sigma$ for all input dimensions $i\in\{1,\dots,d\}$, where $e_{i}$ is the $i^\mathit{th}$ unit vector. We further assume that $\mathcal{I}=[0,1]^d$ and that points in $\mathcal{D}_i$ used for learning $h_i$ are sampled from the uniform distribution on $\mathcal{I}$.

\input{theorem_figure/theorem_fig.tex}

We require that for each hyperplane $h_i$, the fraction of volume removed from $\mathcal{A}_c$ by $h_i$ is not more than a chosen $v\in[0,1]$, i.e., we have $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq v$.
To ensure this, we enforce that for $i\in\{1,\dots,m\}$, the classifier associated with $h_i$ picks its slope parameters $a_{i}$ close to $a_{\kappa(i)}^\text{best}$ for some input dimension $\kappa(i)\in\{1,\dots,d\}$. We quantify the distance between $a_{i}$ and $a_{\kappa(i)}^\text{best}$ in terms of the cosine similarity $\omega_{i} = \frac{\langle a_{i},a_{\kappa(i)}^\text{best}\rangle}{\|a_{i}\|_2\|a_{\kappa(i)}^\text{best}\|_2}$. To enforce the closeness, we assume the existence of a chosen lower bound $\omega_{\min} \in (0,1]$ such that $\omega_{i} \geq \omega_{\min}$ for all $i\in\{1,\dots,m\}$. A possible geometric interpretation of these assumptions is that all classifiers are given imprecise information on $a_{i}^\text{best}$ --- the true slopes of the decision boundaries of $\mathcal{A}_c$, in terms of a maximal error angle $\alpha=\arccos{(\omega_{\min})}$ between them and $e_i$, but no information about the biases $b_{i}^\text{best}$. This is demonstrated in the 2D setting in \figref{fig:theorem23}.

We formally define the maximal width cut in the $k(i)^\text{th}$ dimension of $\mathcal{A}_c$ by a half-space constraint $h_i$, as the solution of the optimization problem $\underset{ x\in\mathcal{A}_c }{\max} \sigma - x[\kappa(i)]$, such that $x$ is missclassified by $h_i$. We denote by $x^{\min}_i$ the value of $x$ for which the maximum is achieved. Next, we aim to analyze and quantify how the uncertainty in $a_{i}$ and $b_{i}$ affects the volume cut from $\mathcal{A}_c$ by the classifier $h_i$.
To this end, we introduce separate error terms $\delta_i$ and $\epsilon_i$ for the maximal width cut in the $\kappa(i)^\mathit{th}$ dimension by deviations in $a_{i}$ and $b_{i}$ from the optimal $a_{\kappa(i)}^\text{best}$ and $b_{\kappa(i)}^\text{best}$, respectively. 

To find the worst-case width $\delta_i$, we search for pairs of points $(p_1,p_2)$, such that $p_1,p_2\in\mathcal{A}_c$ and the property that $p_2$ is correctly classified and $p_1$ is not. Intuitively, as $p_1[\kappa(i)]$ approaches $0$ and $p_2[\kappa(i)]$ approaches $\sigma$, the slope $a_i$ goes further and further away from the optimal $e_i$. Since, the cosine similarity between these vectors is lower-bounded, there exists $p^{\min}_1$ and $p^{\max}_2$ such that $p^{\max}_2[\kappa(i)] - p^{\min}_1[\kappa(i)]$ is maximal. One can look at this difference as the maximum width allowed to be additionally cut in the $\kappa(i)^{th}$ dimension, given that we have ensured some $p^{\max}_2$ close to the decision boundary is correctly classified. Following this intuition, we formally define:
\begin{maxi}
	{p_1,p_2\in \mathcal{A}_c,\; a_{i}\in\reals{d},\; b_{i}\in\reals{}}
	{p_2[\kappa(i)] - p_1[\kappa(i)]}
	{}
	{\delta_{i} = \label{eq:delta_min_lemma}}
	\addConstraint{a_{i} \cdot p_1 + b_i }{\geq0}{}
	\addConstraint{a_{i} \cdot p_2 + b_i }{\leq0}{}
	\addConstraint{\omega_{i}}{ \geq \omega_{\min}}{}.
\end{maxi}
The next lemma shows that the optimization problem defined by \eqref{eq:delta_min_lemma} is independent of $b_i$, as required by our intuitive definition of $\delta_i$, and provides its analytical solution:
\begin{lemma}\label{lm:delta}
	For all $i\in\{1,\dots,m\}$, $\delta_{i}$ is given by the formula
 $\delta_{i} = \sigma\frac{\sqrt{(d-1)\cdot (1 - \omega_{\min}^2)}}{\omega_{\min}}$ and therefore independent of $b_i$.
\end{lemma}
\begin{proof}
	Let $(p^{\min}_1, p^{\max}_2, a_i^{\max}, b_i^{\max})$ be an assignment of values to $p_1$, $p_2$, $a_i$ and $b_i$, respectively, that together maximize $\delta_{i}$. Then, the assignment $(p^{\min}_1 + c \cdot e_{\kappa(i)}, p^{\max}_2+c \cdot e_{\kappa(i)}, a_i^{\max}, b_i^{\max} - c \cdot a_i^{\max}[\kappa(i)])$ also maximizes $\delta_{i}$ for all $c\in\reals{}$ --- that is, the problem is translation invariant in the $\kappa(i)^\mathit{th}$ dimension. Additionally, the hyperplane $a_i \cdot x + b_i = 0$ passes through the points $p^{\min}_1$ and $p^{\max}_2$ that maximize $\delta_{i}$, since otherwise one can choose smaller $p_1[\kappa(i)]$ and bigger $p_2[\kappa(i)]$ until they do, while also improving the objective. Therefore, we can reformulate \eqref{eq:delta_min_lemma} in the equivalent form:
\begin{maxi}
	{p_1,p_2\in \mathcal{A}_c,\; a_{i}\in\reals{d}}
	{p_2[\kappa(i)] - p_1[\kappa(i)]}
	{}
	{\delta_{i} = \label{eq:delta_min_lemma2}}
	\addConstraint{a_{i} \cdot ( p_2 - p_1 )}{=0}{}
	\addConstraint{a_{i}[\kappa(i)]}{ \geq \omega_{\min}}{}
	\addConstraint{\| a_{i} \|_2}{= 1}{,}
\end{maxi}
where the last two constraints come from the definition of $\omega_{\min}$.
We can rewrite $a_{i} \cdot ( p_2 - p_1 )=0$ as \[p_2[\kappa(i)] - p_1[\kappa(i)] = \frac{\sum_{j\in\{1,\dots, d\}\setminus\{\kappa(i)\}}a_{i}[j]\cdot (p_1[j] - p_2[j])}{a_{i}[\kappa(i)]}.\] Since $p_1,p_2\in \mathcal{A}_c$, we know $p_1[j] - p_2[j] \leq \sigma$ for all input dimensions $j\in\{1,\dots,d\}\setminus\{\kappa(i)\}$. The bound is tight and can be achieved for $p_1[j] = \sigma$ and $p_2[j]=0$, for all input dimensions $j\in\{1,\dots,d\}\setminus\{\kappa(i)\}$ independently. Setting $S = \sum_{j\in\{1,\dots, d\}\setminus\{\kappa(i)\}}a_{i}[j]$, we can rewrite \eqref{eq:delta_min_lemma2} as follows:
\begin{maxi}
	{a_{i}\in\reals{d}}
	{\frac{S \cdot \sigma}{a_{i}[\kappa(i)]}}
	{}
	{\delta_{i} = \label{eq:delta_min_lemma3}}
	\addConstraint{a_{i}[\kappa(i)]}{ \geq \omega_{\min}}{}
	\addConstraint{\| a_{i} \|_2}{= 1}{}
\end{maxi}
One can use Lagrangian multipliers to demonstrate that under the conditions in \eqref{eq:delta_min_lemma3}, $S$ is maximized when $a_{i}[\kappa(i)] = \omega_{\min}$ and all other dimension of $a_{i}$ are equal to $\sqrt{\frac{1-\omega_{\min}^2}{d-1}}$. Therefore, $\delta_{i}$ is also maximized under the same conditions and it is given by the formula given in \lemmaref{lm:delta}.
\end{proof}
\lemmaref{lm:delta} demonstrates that $\delta_{i}$ is independent of $i$. For the rest of this section, we refer to its value as simply $\delta$ to simplify the notation.

Let $\epsilon_i$ be the worst-case width cut from the $\kappa(i)^\mathit{th}$ dimension of $\mathcal{A}_c$, for the simple case when $a_{i}$ is optimal ($\omega_{\min}=1$). Since $h_i$ correctly classifies all samples in $\mathcal{D}_i$, $\epsilon_i$ is given by:

\begin{mini}
	{p\in\mathcal{D}_i}
	{\sigma-p[\kappa(i)]}
	{}
	{\epsilon_{i} = \label{eq:eps}}
	\addConstraint{p}{\in\mathcal{A}_c}{.}
\end{mini}

Next, we show that the worst-case width cut, in the general case $\omega_{\min}\leq1$, is given by the sum of $\delta$ and $\epsilon_{i}$:
\begin{lemma}\label{lm:epsilon}
	The worst-case width cut from the $\kappa(i)^\mathit{th}$ dimension of $\mathcal{A}_c$ by the classifier $h_i$ is given by the sum of $\delta$ and $\epsilon_{i}$.
\end{lemma}
\begin{proof}
	Due to the translational invariance property, \eqref{eq:delta_min_lemma}'s solution remains the same if we additionally require $p_2[\kappa(i)]=\sigma - \epsilon_i$. From \eqref{eq:delta_min_lemma}, we know $p_1[\kappa(i)]\geq p_2[\kappa(i)] - \delta_i$. Therefore, $p_1[\kappa(i)]\geq \sigma - \delta_i - \epsilon_{i}$. In other words, the minimal width that cannot be removed from the $\kappa(i)^\mathit{th}$ dimension of $\mathcal{A}_c$, provided $p$ is correctly classified is $\sigma - \delta_i - \epsilon_{i}$. Therefore, the worst-case width that can be cut is at most $\delta_i + \epsilon_{i}$. This bound is tight, as the equality is achieved for the case, where $p$ has all of its coordinates except the $\kappa(i)^\mathit{th}$ equal to $0$.
\end{proof}

Next, we introduce \lemmaref{lm:hp_vol_shrink_lemma}, which quantifies the expected number of samples needed in $\mathcal{D}_i$ to guarantee $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq v$ for a chosen $v\in[0,\frac{\sigma-\delta}{\sigma}]$. 
Note that $v$ cannot be more than $\frac{\sigma-\delta}{\sigma}$, as we cannot guarantee to preserve more than $\sigma - \delta$ of the width in the $\kappa(i)^{th}$ dimension under any $\epsilon_i\in[0,\sigma]$ owing to the uncertainty in the estimation of slopes $a_i$.

\begin{lemma}\label{lm:hp_vol_shrink_lemma}
For $v\in[0,\frac{\sigma-\delta}{\sigma}]$ and $i\in\{1,\dots,m\}$, the expected number of samples $n_s =\expect[|\mathcal{D}_i|]$ until $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq v$ holds is $n_s =\frac{1}{\sigma^d\left( 1-\frac{\delta}{\sigma}-v\right)}$ in the worst case.
\end{lemma}
\begin{proof}
We look at the probability of a point $p$ to be contained $\mathcal{D}_i$, such that $p[\kappa(i)] \geq \sigma - \epsilon$ for a given $\epsilon\in[0,\sigma]$. When such point exists, we know $\epsilon_i\leq \epsilon$. That is, for a given $\epsilon\in[0,\sigma]$, we are interested in the probability of sampling a point in the hyperrectangle $\prod^{d}_{i=1}[s_i,\sigma]$ with $s_i = 0$ for all dimensions $i\in\{1,\dots,d\}\setminus\{\kappa(i)\}$ and $s_{\kappa(i)}=\sigma-\epsilon$. Since we sample $\mathcal{D}_i$ from the uniform distribution on $\mathcal I$, the probability is given by the ratio of the volumes of $\mathcal{I}$ and the hyperrectangle, which has volume $\sigma^{d-1}\epsilon$. Therefore, the probability of sampling $p$ is $\sigma^{d-1}\epsilon$ and the expected number of samples $n_s$ to get such point $p$, which is a geometrically distributed random variable, is $\frac{1}{\sigma^{d-1}\epsilon}$.

From \lemmaref{lm:epsilon}, we know that $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq \frac{ \sigma - \epsilon_{i} - \delta}{\sigma}\geq \frac{ \sigma - \epsilon - \delta}{\sigma}$, since at least $\sigma - \epsilon - \delta$ portion of the width of $\kappa(i)^\mathit{th}$ dimension of $\mathcal{A}_c$ cannot be removed by $h_i$. Therefore, if we choose $\epsilon = \sigma - \delta - v \sigma$, we can guarantee $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq v$. Plugging our choice of $\epsilon$ we conclude that $n_s=\frac{1}{\sigma^d(1-\frac{\delta}{\sigma}-v)}$ is the worst-case expected number of points we need to sample to obtain $h_i$, such that $\frac{\vol(h_i \cap \mathcal{A}_c)}{\vol(\mathcal{A}_c)} \geq v$ holds.

\end{proof}

Next, we generalize this result to the full region $\mathcal{P}$:
\begin{theorem}\label{th:hp_vol_shrink_theorem}
	For all $V\in[0,\left(\frac{\sigma-\delta}{\sigma}\right)^{m}]$ the expected number of samples $n_s =\expect[|\mathcal{D}_i|]$, such that $\frac{\vol(\mathcal{P})}{\vol(\mathcal{A}_c)} \geq V$ holds is at most $n_s =\frac{1}{\sigma^d\left(1-\frac{\delta}{\sigma}-V^{\frac{1}{m}}\right)}$.
\end{theorem}
\begin{proof}
	Applying \lemmaref{lm:hp_vol_shrink_lemma} with $v = V^\frac{1}{m}$ for all half-space constraints in $\mathcal{P}$ and multiplying the individual volume bounds together we obtain the required result.
\end{proof}



In the next theorem, we consider the even simpler setting of $\omega_{\min} = 1$ -- that is the setting in which our binary classifiers only considers axis-aligned half-space constraints. We also assume the datasets $\mathcal{D}_i$ are collected uniformly at random from $\mathcal{P}_i$. We demonstrate that ensuring that $\mathcal{P}$'s volume shrinks by certain amount becomes more difficult as $\mathcal{P}$ approaches $\mathcal{A}_c$:
\begin{definition}
For all $i\in \{0,\dots ,m$\} corresponding to the polyhedra sequence $\mathcal{P}_i$, and all input dimensions $k\in \{1,\dots ,d\}$, we call  $u^k_i=\underset{x\in \mathcal{P}_i}{\max}( x[k] )$ the upper bound of dimension $k$ in $\mathcal{P}_i$.
\end{definition}
\begin{theorem}\label{th:it_progress_theorem}
For all $i\in \{0,\dots ,m-1$\} corresponding to the polyhedra sequence $\mathcal{P}_i$, for which $u^{\kappa(i+1)}_i > \sigma$ and for all $v\in(0,1]$, the expected number of samples $n_s=\expect[|\mathcal{D}_{i+1}|]$ needed to create $h_{i+1}$ such that $\frac{u^{\kappa(i+1)}_{i+1}-\sigma}{u^{\kappa(i+1)}_{i}-\sigma}\leq v $ holds is $n_s=\frac{u^{\kappa(i+1)}_i}{(u^{\kappa(i+1)}_i-\sigma)\cdot v}$. Here, the quantity $\frac{u^{\kappa(i+1)}_{i+1}-\sigma}{u^{\kappa(i+1)}_i-\sigma}$ quantifies the shrinking in the $\kappa(i+1)^{th}$ dimension in step $i+1$.
\end{theorem}
\begin{proof}
	We show a depiction of our proof of \thref{th:it_progress_theorem} in the 2D setting in \figref{fig:theorem24}. We consider $\kappa(i+1)^\mathit{th}$ dimension of $\mathcal{A}_c$ (the horizontal dimension in \figref{fig:theorem24}). Similarly to \lemmaref{lm:hp_vol_shrink_lemma}, we quantify the probability that there exists a negative sample $p\in\mathcal{D}_h$ such that its $\kappa(i+1)^\mathit{th}$ dimension has a coordinate in $ [\sigma,(u^{\kappa(i+1)}_i-\sigma)\cdot v + \sigma]$. \figref{fig:theorem24} depicts the region of possible locations for $p$ as an orange rectangle. We know that if such point $p$ exists, due to the assumption $h_{i+1}$ correctly classifies all samples the condition $\frac{u^{\kappa(i+1)}_{i+1}-\sigma}{u^{\kappa(i+1)}_{i}-\sigma} \leq v$ holds. Since $\mathcal{D}_{i+1}$ is uniformly sampled from $\mathcal{P}_i$ the probability of sampling such $p$ is given by the ratio of the volumes of the orange region and $\mathcal{P}_i$. This probability is $\frac{(u^{\kappa(i+1)}_i-\sigma) \cdot v}{u^{\kappa(i+1)}_i}$. The number of samples need for $p$ to exist is geometrically distributed and its expectation is given by $n_s=\frac{u^{\kappa(i+1)}_i}{(u^{\kappa(i+1)}_i-\sigma)\cdot v}$.
\end{proof}





==> theory_implication.tex <==
\section{Practical Implications of our Theoretical Results}
We next discuss the impact of our theoretical results in the previous section on the design of our algorithms. 
\thref{th:hp_vol_shrink_theorem} demonstrates that despite our simplifying assumptions it is computationally expensive to create $\mathcal{P}$ for high values of $d$ or $V$.
It can also be seen that small inaccuracies in the estimated half-space constraint slopes can lead to big portions of the volume being cut. In particular, we see that the quantity $(\frac{\sigma-\delta}{\sigma})^{m}$ acts like an upper bound on the volume of $\mathcal{A}_c$ that can be guaranteed to be kept. For example with $d=m=10$, and a slope difference of only up to $4\degree$, the upper bound on the volume guaranteed to be kept is $V \approx 0.9$. For $d=m=100$ and the same upper bound on the volume, the maximum slope difference allowed is only $\approx 0.12\degree$. Last but not least, we see that the algorithm is particularly sensitive to $V$ especially in high dimensions -- e.g. for $d=m=100$, $\sigma=0.8$, $\frac{\sigma-\delta}{\sigma}=1$ increasing $V$ from $0.9$ to $0.95$ doubles the number of samples required at each iteration from $\approx 4.7 \times 10^{12}$ to $\approx 9.6 \times 10^{12}$. We further note that the above results assume that there is an exact procedure to determine whether a given region is adversarial. Exact verifiers for neural networks do not scale on the sizes of networks considered in our experiments, therefore we actually use inexact verifiers in our algorithms for scalability which can make the problem even harder. Overall, for the general case encountered in our experiments, where $\mathcal{A}_c$ can be an arbitrary connected shape and inexact verifiers are used, the complexity of sampling would be at least as hard as our results.

Since computing optimal regions is computationally expensive, we use heuristics to preserve as much of $\mathcal{A}_c$ as possible in our algorithms presented in \secref{sec:framework}. 
In \thref{th:hp_vol_shrink_theorem}, $n_s$ is inversely proportional to the quantity $\sigma^{d}$ which suggests that the effort of constructing a precise $\mathcal{P}$ is less when
the volume of $\mathcal{A}_c$ is close to that of $\mathcal{I}$. Therefore, we start with an input region $\mathcal{I}$ such that the ratio $\frac{\vol(\mathcal{A}_c)}{\vol(\mathcal{I})}$ is not too low by estimating tight bounding boxes around $\mathcal{A}_c$ before initiating the half-space generation portion of our algorithm (\secref{sec:initcandidates}). 
 As per \thref{th:hp_vol_shrink_theorem}, the amount of incorrectly removed volume grows with the angle between the hyperplane $h_i$ and the decision boundary, our sampling procedure in \secref{sec:counter} employs heuristics so this angle is small.  

From \thref{th:it_progress_theorem} for a constant $v$ it follows that  $\underset{u^{\kappa(i+1)}_i\to \sigma}{\lim}n_s = \infty$. Therefore, with each new half-space it becomes harder and harder for a general sampling algorithm to progress. Another way to look at \thref{th:it_progress_theorem} is that for a constant number of samples $n_s$ the guaranteed volume removed from $\mathcal{P}_i$ goes to $0$ as $i \to \infty$. This theoretical prediction is consistent with what we observe in practice, where our algorithm sometimes will take a lot of iterations to converge. In \secref{sec:shrink}, we propose a shrinking procedure to deal with this issue.

